Network-aware Recommender System via Online Feedback Optimization

Personalized content on social platforms can exacerbate negative phenomena such as polarization, partly due to the feedback interactions between recommendations and the users. In this paper, we present a control-theoretic recommender system that explicitly accounts for this feedback loop to mitigate polarization. Our approach extends online feedback optimization - a control paradigm for steady-state optimization of dynamical systems - to develop a recommender system that trades off users engagement and polarization reduction, while relying solely on online click data. We establish theoretical guarantees for optimality and stability of the proposed design and validate its effectiveness via numerical experiments with a user population governed by Friedkin-Johnsen dynamics. Our results show these "network-aware" recommendations can significantly reduce polarization while maintaining high levels of user engagement.

==> oldstuff.tex <==
%%Problem Formulation:

Given an input/output system, an input $u\in\mathbb{R}^n$ is \emph{persistently exciting} for the system if the corresponding Henkel matrix has full rank, i.e., there exists $S\in \mathbb{N}$ such that
\begin{equation*}
     \mathrm{Rank}[\Delta u^{{t-S-1},{t-S-2}},\Delta u^{{t-S},{t-S-1}},\ldots,\Delta u^{{t},{t-1}}] = n,
\end{equation*}
where $\Delta u^{t_1,t_2} := u^{t_1} - u^{t_2}$.
\gb{old section}
\begin{figure}
    \centering
    \includegraphics[scale=0.5]{Figures/blockdiagram_1.jpg}
    \caption{Closed loop representation between the opinion dynamics and the recommender as an OFO algorithm.}
    \label{fig:blockdiagram_1}
\end{figure}
In this work, we consider the closed-loop between opinion dynamics and recommender systems by designing the recommender as an OFO algorithm, as in Fig. \ref{fig:blockdiagram_1}. The system dynamics is represented as:
\begin{align} 
    x({k+1}) & = f(x(k),p(k),d(k)), \notag \\
    \Bar{c}(k) & = g(p(k),x(k)), 
\end{align}
where, $x(k),p(k),d(k)\in[-1,1]^n$ and $\bar{c}(k)\in [0,1]^n$, $\forall\, k\in\mathbb{N}$. Moreover, $f(\cdot,\cdot,\cdot): ([-1,1]^n)^3\mapsto [-1,1]^n$ and $g(\cdot,\cdot):([-1,1]^n)^2\mapsto [0,1]$ represent the opinion dynamics and clicking behaviour of the users, respectively. Here, $x_i(\cdot),p_i(\cdot)$ represent the opinion of  user $i$, $i\in[n]$ and the position of the article provided to the user $i$ by the recommender, respectively. We assume there is one single topic of discussion on the platform. The issue is assumed to be polarizing, e.g. abortion, so that a position $+1$ ($-1$) can be interpreted as a news strongly in support of (against)  the issue. Finally, $d(\cdot)$ represents an influence external to the platform that affects opinions, e.g. television, that could be interpreted as a disturbance to the system, and $\bar{c}_i(\cdot)$ is the clicking ratio of the user $i$ on the news over a time horizon. Namely, if  $c(k)\in\{0,1\}^n$ indicates if the user clicked ($c=1$) or not $(c=0)$ on a news article with position $p'$ at time instant $k$, then, by indicating as $\mathcal{J}(p')$ the set of the time indices in which $p'$ has been provided, $\bar{c}(k) = \frac{1}{|\mathcal{J}(p')|}\sum_{j\in \mathcal{J}(p')}c(j)$. \gb{This should be a function of $p(k)$ and $x(k)$ only, $g(p,k)$.}

The positions $p$ are provided by the recommender system to the users by solving the following non-convex optimization problem:
\begin{align} 
    \underset{p}{\mathrm{min}} \ &  \phi(p,x), \\
    \textrm{s.t} \  x & = h(p,d), \nonumber\\ 
    p &\in \mathcal{P}. \nonumber 
\end{align}
The recommender system aims to maximize user engagement. For this reason, we consider the cost function as the sum of the clicking ratio $\Bar{c}$ of the $n$ users in the social network, namely $\phi(p,x) := -1_n^\top g(p,x)$.

By following the approach from OFO, the optimization problem \eqref{opt} is solved, assuming that the opinions have reached a steady-state condition $x = h(p,d)$, and is subject to a budget constraint over the positions. Namely we require the positions to be in $\mathcal{P}$, with $\mathcal{P} := \{p \ \in \mathbb{R}^n : |p_i| \leq 1 \ \forall i \in [n], ||p||_1 \leq \kappa\}$, with $\kappa> 0$ a constant and $|p_i|$ the advertisement cost associated with the recommendation of position $p_i$ to user $i$. This constraint models the fact that the space over a social network is costly.

The goal of the recommender system is to find a $p^{*}$ to increase the likelihood of the users clicking on the articles provided on the platform by solving the optimization problem \eqref{opt}. The problem we aim to address presents three main challenges:
\begin{enumerate}
    \item The real-time user opinions $x(k)$ are unavailable $\forall k\in\mathbb{N}$ to the recommender system. The only online information available is the user's clicks $c(k) \in \{0,1\}^n$ on the provided articles (\textit{implicit feedback}).
    \item The process model $f(x,p,d)$ is unknown. Hence the steady-state map $h(p,d)$ is also unknown.
    \item The clicking behaviour $g(p,x)$ of the users is unknown.
\end{enumerate}
In addition to the above three, there is also a time-scale separation issue between opinions and recommendations since they evolve on time scales similar in magnitude, resulting in sub-optimal $p^{*}$.

To make problem \eqref{opt} more tractable, we will operate under some regularity assumptions over the cost function and the dynamics that are formalized in the following.
\begin{assumption}[Cost Function]\label{costfunctionassumption} $\phi(p,x)$ is $L_p,L_x$-smooth with respect to $p,x$, respectively.
\end{assumption}
With the above assumption, we state that although unknown, the {clicking behaviour} of the users does not abruptly change with respect to either opinions or positions.
\begin{remark}[Well-posed Dynamics] \label{wellposedness}
The opinion dynamics $x({k+1}) = f(x(k),p(k),d(k))$ is forward-invariant in the set $[-1,1]^n:x(k) \in [-1,1]^n \  \forall \ k\in\mathbb{N} \iff x(0) = x_0 \in [-1,1]^n$, when $p(k),d(k)\in[-1,1]^n\forall k\in\mathbb{N}$.
\end{remark}
\begin{assumption}[Local steady state] \label{localSS}
For every $p$, there exists a unique steady-state opinion vector $x$. Further, for every $p$, the dynamics \eqref{opmodel} admits at least one instant where local steady-state behaviour is observed. 
\end{assumption}
Assumption \ref{localSS} guarantees that a stable equilibrium $x=h(p,d)$ exists and is bijective with respect to $p$. However,
for asymptotic convergence of $p$, stability on the dynamical system is a necessary but not sufficient condition \cite{colombino,hauswirth1}.

% Proofs
\begin{proof}\label{Lsmooth_fullproof}
    For any $p_1,p_2\in\mathbb{R}^n$ and $x_1 = h(p_1,d),x_2 = h(p_2,d)$, we have:
    \footnotesize
    \begin{align*}
        ||\Phi(p_1) - \Phi(p_2)|| \leq & ||\nabla_p\phi(p_1) - \nabla_p\phi(p_2)|| + ||H|| \ ||\nabla_x\phi(x_1) - \nabla_x\phi(x_2)|| +  \\
        & ||H^\top|| ||\nabla_x\psi(x_1) - \nabla_x\psi(x_2)||\\
        \underset{(a)}{\leq} & L_p||p_1-p_2|| + LL_x||x_1-x_2||\\
        \underset{(b)}{\leq} & (L_p + L^2L_x)||p_1-p_2||.
    \end{align*}
    \normalsize In $(a)$, we use Assumption \ref{costfunctionassumption}, i.e. $\phi$ is $L_p,L_x-$smooth with respect to $p,x$, respectively. Further, we use Assumption \ref{SSmapassumption}, i.e. the steady-state map being $L-$Lipschitz, thus $||H||\leq L$. In $(b)$, we again use Assumption \ref{SSmapassumption}, with $x_1 = h(p_1,d)$ and $x_2=h(p_2,d)$ for some disturbance $d\in[-1,1]^n$.
\end{proof}

% Study-2 results

\subsubsection{Impact of Prejudice on Recommendations}\label{study2}
In this sub-section, we discuss the effects of the external influence $d(k)$ on recommendations. In particular, we shed light on the trade-offs that the recommender makes between prioritizing influencers and stubborn users. We analyze method $M_5$ with budget constraint $\kappa=7$ and all the users following clicking behaviour $C_A$. The FJ model considered in this section is different from that considered in the previous one.

The extended FJ model in \eqref{FriedkinJohnsen} dictates that the opinions of the users are not only subject to interactions in the network but also to their own prejudices and recommendations. Thus, by incorporating budget constraints, we expect that not all recommendations will be prioritized for users with high node centrality. Some recommendations would also be provided to stubborn users or users holding a higher trust in the news article (recorded by $\Gamma_p$) in the hope of maximizing the overall clicking rate.
\begin{figure}
    \centering
    \includegraphics[scale=0.21]{Figures/study2_influencerbudget.jpg}
    \includegraphics[scale=0.23]{Figures/study2_costs.jpg}
    \caption{Comparison of (a) (left) Budget allocated to influential users and (b) (right) Performances using final average clicking ratio, with varying degrees of stubbornness. The budget constraint is $\kappa=7$.}
    \label{fig:study2comparisonsA}
\end{figure}

In Fig. \ref{fig:study2comparisonsA}(a), we record the influencer budget, which we define as the recommendations provided to $\lfloor\kappa\rfloor$ users who hold high influence in the graph, i.e. $\sum_{j\in\mathcal{K}}|p_j^{*}|$, where $\mathcal{K}$ refers to a set of the first $\lfloor\kappa\rfloor$ users among the $n$ with the largest column-sum in $A$. In Fig. \ref{fig:study2comparisonsA}(b), we record the performance of our algorithm (final mean clicking ratio) across 20 Monte Carlo trials as the external disturbance is increased from $\mathbb{E}\big[d(k)\big]=0$ to $x(0)$.

\textit{The social network plays a smaller role in the case of more prejudiced users}. In Fig. \ref{fig:study2comparisonsA}(a), as the prejudice factor is reduced, we observe an increase in recommendations provided to the $\kappa$ most influential users. This is owing to the stubbornness factor being reduced, leading to the users being more inclined towards others' opinions. The OFO recognizes this and prioritizes the social network more than an individual's prejudice. However, there seems to be an exception when $\mathbb{E}\big[d(k)\big]=0$. This occurs because the influencers themselves do not hold strongly to their initial opinions. Thus, prioritizing recommendations towards them need not necessarily lead to the best performance.

\textit{The consideration of the social network leads to an increase in clicking ratio, even when the users are not prejudiced.} As seen in Fig. \ref{fig:study2comparisonsA}(b), a higher prejudice leads to more effective recommendations, which was already observed in \cite{rossi} for clicking behaviour $C_A$. If the network were not considered, then personalization alone would have been used to provide recommendations, which is difficult to ascertain as the prejudice factor is zero. This indicates an \textit{advantage of network awareness through sensitivity estimation, as opposed to decoupled recommendations}. More on this comparison is provided in the next sub-section.
\begin{figure}
    \centering
    \includegraphics[scale=0.21]{Figures/study2_xf.jpg}
    \includegraphics[scale=0.21]{Figures/study2_varxf.jpg}
    \caption{Comparison of (a) (left) Average final opinions and (b) (right) Variance of the final opinions, with respect to varying degrees of stubbornness.}
    \label{fig:study2comparisonsB}
\end{figure}

In Fig. \ref{fig:study2comparisonsB}, on varying $\mathbb{E}\big[d(k)\big]$, we compare the average final opinions ($\sum_{i=1}^n x_i^{*}/n$) and their variance ($||x^{*} - \frac{1}{n}\sum_{i=1}^n x_i^{*}1_n||^2$), with the latter often being used as a measure for polarization \cite{musco2021quantify}. For the model considered in this section, the initial average opinion is found to be $\sum_{i=1}^n x_i(0)/n = -0.25$. The initial polarization level is found to be $4.17$. Although Fig. \ref{fig:study2comparisonsB} indicates that for all levels of stubbornness, the final polarization level has reduced, this is at a cost of the user's swinging to position "$-1$". Thus, with the users following clicking behaviour $C_A$, \textit{above a certain level of stubbornness, the recommendations provided to the users are more inclined towards the majority stance in the network held initially, leading to the formation of echo chambers}.

Overall, Fig. \ref{fig:study2comparisonsA},\ref{fig:study2comparisonsB} indicate that by performing disturbance rejection on the external influence $d(\cdot)$, one can design recommenders that could establish a trade-off between recommendations that attract a higher clicking ratio in the interest of the content creator, and lowering polarization and promoting social interactions, in the interest of a humane society. A possibility of carrying this out in the context of OFO would be by including output constraints \cite{verena} to limit extreme opinions.


\begin{algorithm}
\caption{$\Bar{c}^{*}$ = $\textrm{RossiRecommender}[N,T,n,\kappa,\epsilon]$} \label{alg:rossirecommender}
    \begin{algorithmic}
    \STATE Select $\lfloor\kappa\rfloor$ users at random out of $n$: Selected user set $\mathcal{U}$
    \STATE For users $i \notin \mathcal{U}$, $p_i(k)=0, \forall k\in\mathbb{N}$
    \STATE $p(0)\leftarrow 0_n$
    \STATE For users $i\in\mathcal{U}, P(p_i(1)=+1)=P(p_i(1)=-1)=0.5$
    \FOR{$k\in [2,N]$}
        \STATE Collect clicks $c(k)$ from users
        \FOR{$i\in\mathcal{U}$}
            \STATE $r_i^{+}(k-1) \leftarrow \# (p_i(t)=+1), t\leq k-1$
            \STATE $r_i^{-}(k-1) \leftarrow \# (p_i(t)=-1), t\leq k-1$
            \STATE  $c_i^{+}(k-1) = c_i(t)$ when $p_i(t)=+1$, $\forall t\leq k-1$ 
            \STATE  $c_i^{-}(k-1) = c_i(t)$ when $p_i(t)=-1$, $\forall t\leq k-1$ 
            \STATE Positive clicking ratio $\Bar{c}_i^{+}(k-1) \leftarrow \frac{\sum_{t=0}^{k-1}c_i^{+}(t)}{r_i^{+}(k-1)}$
            \STATE Negative clicking ratio $\Bar{c}_i^{-}(k-1) \leftarrow \frac{\sum_{t=0}^{k-1}c_i^{-}(t)}{r_i^{-}(k-1)}$
            \STATE Assign $p_i(k)$ using decision rule in \eqref{rossidecisionrule}
        \ENDFOR
    \ENDFOR
    \RETURN $\Bar{c}^{*} \leftarrow \sum_{k=N-T+1}^N ||c(k)||_1/(nT)$
    \end{algorithmic}
\end{algorithm}

Based on Assumption \ref{POEassumption}, we have the following remark:
    \begin{remark}[Uniform Complete Observability] \label{POEinequality}
    An immediate consequence of Definition \ref{POEhenkel} is that there exists a $T$ large enough and an $\alpha>0$ \textcolor{red}{$\alpha?$}such that 
    \begin{equation} \label{deltapbound}
        \alpha_1 I_n \leq \sum_{l=0}^{T} \Delta p(\tau_{i-l},\tau_{i-l-1}) \Delta p(\tau_{i-l},\tau_{i-l-1})^\top \leq \alpha_2 I_n.
    \end{equation}
    \end{remark}
    With $\alpha_1>0$, uniform complete observability \cite{picallo} \textcolor{red}{what do you mean by observability? What is the output and what is the state?} of the measurement model in \eqref{measurementmodelKF} is guaranteed \cite[Chapter 7]{andrew}\textcolor{red}{is there any online version of this book? I cannot find it}. Further, since $\sigma_q(k)>0 \ \forall k\in\mathbb{N}_0$ from \eqref{sigmaq}, we have $Q(k)>0 \ \forall k\in\mathbb{N}_0$, leading to uniform complete controllability.

    There exists an upper-bound on the state estimation error according to \eqref{upperbound_ANN_x}. Further, in \eqref{KFposterior_state}, the posterior update is projected onto a polyhedra $\mathcal{H}$, making the projection non-expansive. Moreover, since we have established that the process and measurement model for sensitivity learning are completely observable and controllable, exponential convergence on the variance of the sensitivity estimation error is guaranteed, i.e. $\exists C_1,C_2>0, \alpha\in(0,1): \mathbb{E}[||e(k)||^2]\leq C_f + C_1\alpha^{C_2k}$. \textcolor{red}{what is this????}


    This chapter discusses the learning and control techniques for designing the recommender as an optimization algorithm. The solution to the optimization problem in \eqref{opt} is given by the following projected gradient descent rule, solved online:

\footnotesize{
\begin{equation}
    p({k+1}) = \mathbb{P}_\mathcal{P}\Bigg[p(k) - \eta \begin{pmatrix}
        I_n & H(k)^\top
    \end{pmatrix}
    \begin{pmatrix}
        \nabla_p\phi(p(k),x({k+1}))\\
        \nabla_x\phi(p(k),x({k+1}))
    \end{pmatrix}\Bigg].
\end{equation}}
\normalsize Here, $\mathbb{P}_\mathcal{P}[\cdot]$ is the Euclidean projection onto the polyhedra $\mathcal{P}$, and  $\eta$ is the step-size. The term $H(k) := \nabla_p h(p(k),d(k))$ is defined as the sensitivity and arises from chain-rule of the derivative of the cost function $\phi(p,x)$ with respect to $p$. Further, we approximate the steady-state values $x$ with its real-time measurements $x({k+1})$, assuming sufficient time-scale separation \cite{picallo}. A special advantage of OFO is that, unlike offline feed-forward methods, the steady-state model need not be known, and only the sensitivity is required \cite{hauswirth2021optimization}.
\begin{figure}
    \centering
    \includegraphics[scale=0.5]{Figures/blockdiagram_2.jpg}
    \caption{Representative block diagram of the overall proposed recommender system design.}
    \label{fig:blockdiagram_2}
\end{figure}

Fig. \ref{fig:blockdiagram_2} represents the overall design of the recommender in closed-loop with the opinion dynamics of the users. The three challenges mentioned in Section \ref{sec:problemformulation}, namely unknown opinions, network topology \textcolor{red}{you didn't mention this as a challenge before} and clicking behaviour correspond to real-time states $x(k+1)$, sensitivity $H(k)$ and the cost function $\phi(p,x)$  along with its gradients $\nabla_p\phi,\nabla_x\phi$ in the gradient descent rule in \eqref{PGD_ones} to be unknown.

To address these challenges, we now divide the solution approach into three levels. Level 1 is concerned with opinion and clicking behaviour estimation. Level 2 is concerned with sensitivity estimation. Level 3 is associated with gradient estimation and optimization. \textcolor{red}{link level 1,2,3 with the challenges above}

We stress that the only online information available to the recommender system is the ratio $\Bar{c}$ of clicks of the users over the news provided to them. In Level 1, we develop a black-box model that describes the clicking behaviour $g(p,x)$ in \eqref{opmodel}. Using supervised learning techniques, we then estimate the opinions $\hat{x}$ from the clicking ratio and the positions. In Level 2, we have a periodic trigger mechanism that ensures time-scale separation between the opinion dynamics and the news provider.  Once triggered, new sensitivity estimates are generated online using a Kalman filter and provided to the OFO rule in \eqref{PGD_ones} \textcolor{red}{you didn't call this ofo rule before, be consistent}. Subsequently, in Level 3, new positions are sent to the users using the OFO rule in \eqref{PGD_ones}, where the gradients $\nabla_x\phi,\nabla_p\phi$ are computed numerically using the finite forward difference method \cite{katya}. In the following sections, we describe the three levels in detail.


\subsection{Lemma \ref{sensitivityconstraint}}
\label{sensitivityconstraintproof}
%\textcolor{red}{Assume FJ Dynamics from the beginning by writing it in the statement. You cannot have a general statement and make the proof for a particular case. Also, requiring row-stochastic gradient is very unrealistic}\textcolor{green}{Without assuming some form for the opinion dynamics, it's not possible to prove this lemma. But, I am very sure that this lemma would hold true for any opinion dynamics. I don't want to assume FJ from the beginning as I fear this may reduce the scope of our work.}
\textcolor{green}{to be removed}
\begin{lemma}[Sensitivity Constraint]\label{sensitivityconstraint}
    The entries of the sensitivity lie in $[0,1]$, i.e. $\nabla h(p,d)_{ij}^k\in[0,1],\forall i,j\in[n],\forall k\in\mathbb{N}_0$.
\end{lemma}
\begin{proof}
We prove this lemma by assuming the following structure for the opinion dynamics:
    \begin{equation}\label{generaldynamics}
        x^{k+1} = (I_n - \Gamma_p - \Gamma_d)f_x(x^k) + \Gamma_p f_p(p^k) + \Gamma_d f_d(d^k).
    \end{equation}
    \normalsize We now discuss some assumptions and remarks on the above model. With the above dynamics, we state that the opinions evolve as a convex combination of the opinions of all the users in the network, positions and external disturbances. Since the dynamics is forward invariant in $[-1,1]^n$ (Assumption \ref{ass:ODasm}), we must have $f_x(\cdot),f_p(\cdot),f_d(\cdot)\in[-1,1]^n$ and $\Gamma_p + \Gamma_d \leq I_n$. Further, we assume that all the users in the network are susceptible to recommendations: $\Gamma_p>0$.
    
    For local stability about $(x,p,d)$, we assume that the Jacobian matrix $\nabla_x f_x(x)$ is row sub-stochastic, i.e. $\nabla_x f_x(x) 1_n \leq 1_n$ and $\big(\nabla_x f_x(x)\big)_{ij}\in[0,1], \forall i,j\in[n]$, leading to $\rho\big((I_n-\Gamma_p-\Gamma_d)\nabla_x f_x(x)\big)<1$, where $\rho(\cdot)$ is the spectral radius. Further, according to Assumption \ref{ass:ODasm}, we must have $\nabla_p f_p(p)\in[0,1]^{n\times n}$. We also assume that $x_i(k+1) = f_i(x(k),p_i(k),d_i(k))$, making $\nabla_p f_p(p)$ a diagonal matrix with $\nabla_p f_p(p)\in\mathcal{D}_{[0,1]}^n$.

    The steady-state condition at $(x,p,d)$ in \eqref{generaldynamics} is:
    \begin{equation*}
        x - (I_n - \Gamma_p - \Gamma_d)f_x(x) - \Gamma_pf_p(p) - \Gamma_df_d(d)=0.
    \end{equation*}
    \normalsize We call this map as $\psi(p,x,d)=0$. The sensitivity $H:= \nabla_p h(p,d)$ from the steady-state map $x=h(p,d)$ can be obtained using the implicit function theorem (Thm. 1.B.1, \cite{implicitfunctions}) as $H := -\nabla_x\psi(p,h(p,d),d)^{-1}\nabla_p\psi(p,h(p,d),d)$. \normalsize Thus, we obtain the sensitivity as $H = (I_n - \Tilde{f})^{-1}\Gamma_p\nabla_pf_p(p)$, where $\Tilde{f} = (I_n - \Gamma_p - \Gamma_d)\nabla_xf_x(h(p,d))$.

    We now prove that the sensitivity entries are non-negative. The matrix $(I_n - \Tilde{f})$ is non-singular, thus, we write $H = \big(\sum_{l=0}^\infty \Tilde{f}^l\big)\Gamma_p\nabla_pf_p(p)$. Since $\nabla_xf_x(h(p,d))$ is row sub-stochastic and $(I_n - \Gamma_p - \Gamma_d) \in \mathcal{D}_{[0,1)}^n$, $\Tilde{f}$ is non-negative, leading to $\Tilde{f}^l$ being non-negative $\forall l\geq 0$. Further, $\Gamma_p\in \mathcal{D}_{(0,0.5]}^n$ and $\nabla_p f_p(p)\in\mathcal{D}_{[0,1]}^n$, leading to $H_{ij}\geq0 \forall i,j\in[n]$.

    We now show the upper bound on the sensitivity entries. Let $D := (I_n - \Tilde{f}^\top)^{-1}$. By the matrix inversion lemma \cite{matrixinversionlemma}, we write $D^\top = \Tilde{A}D^\top + I_n$ and $D_{ii}= 1 + \sum_{j=1}^n \Tilde{f}_{ij}D_{ij}$. Since $\Tilde{f}$ is row sub-stochastic, $D$ is diagonally dominant (Thm. 1, \cite{puhalskii2018properties}) in its rows, leading to $D_{ij}\leq D_{ii}, \forall i,j\in[n]$. Thus, we write $D_{ii}\leq 1 + D_{ii}\sum_{j=1}^n \Tilde{f}_{ij}$. Since $\Tilde{f}:= (I_n - \Gamma_p - \Gamma_d)\nabla_xf_x(h(p,d))$ and $\nabla_xf_x(h(p,d))$ is row sub-stochastic, we have  $\sum_{j=1}^n \Tilde{f}_{ij}\leq 1 - (\Gamma_p)_{ii} - (\Gamma_d)_{ii}, \forall i\in[n]$. We note that the sensitivity is $H^\top=D^\top\Gamma_p\nabla_pf_p(p)$. Since $D_{ij}\leq D_{ii}$, $D_{ii}\leq 1/((\Gamma_p)_{ii}+(\Gamma_d)_{ii})$ and $\nabla_p f_p(p)\in\mathcal{D}_{[0,1]}^n$, we obtain $H_{ij}\leq (\Gamma_p)_{jj}/((\Gamma_p)_{jj}+(\Gamma_d)_{jj})\leq 1,\forall i,j\in[n]$. 
\end{proof}

